Type-II Seesaw Higgs triplet productions and decays at the LHC

The Type-II Seesaw Model provides an attractive scenario to account for Majorana-neutrino masses. Its extended Higgs sector, if sufficiently light, can have a rich and distinctive phenomenology at the LHC while yielding automatically an essentially Standard-Model-Higgs-like state. Several phenomenological studies have been devoted to the scalar sector of this model, as well as experimental searches focusing mostly on the (doubly-)charged states. In this paper we present an exhaustive study of the main production and decay channels of all the non-standard scalar states originating from the $SU(2)_L$ doublet and a complex triplet of the model. We stick to scenarios where lepton-number-violating decays are suppressed, for which present experimental limits are still weak, highlighting theoretical parameter sensitivities that were not previously emphasized in the literature and the uncertainties they can induce for the experimental searches at the LHC. A comprehensive classification of the various cascade decays and corresponding Standard Model particle multiplicities is provided. As an illustration, a detailed prospective search study at the LHC with an ATLAS-like detector is carried out on some benchmark points, for charged, doubly-charged, and, for the first time, neutral state productions

==> tables/Charged_finalstates.tex <==
%%%%%
%%%%%
%%%%%
\begin{table}[ht!]
\centering
\def\arraystretch{1.2}
 \caption{ 
    The most promising final states for the charged $H^{\pm \pm} H^{\mp}$ associated production sector for $m_{H^{\pm \pm}} = 220, 300, 400$~GeV and  $\sin\alpha = $ $1 \times 10^{-4}$, $8 \times 10^{-4}$ and  $1.2 \times 10^{-3}$ values.
}
\label{tab:charged_finalstates}
\scalebox{0.65}{
\begin{tabular}{ c |c c c c c c c c c c c c  }
\hline \hline
& 2j & 2j+MET & 4j & 4j+MET & 6j & 6j+MET & 8j & 8j+MET & 10j & 10j+MET & 12j & 12j+MET \\
\hline 
1l & & & & & & 2b & & 0b, 2b & & 0b, 2b & & 2b \\
2l & & & & 2b & & 0b, 2b & 0b, 2b & 0b,2b &0b & 0b,2b & 0b & \\
3l & & 2b &  & 0b,2b & & 0b,2b & & 0b,2b & &0b & & \\
4l  & & 0b & & 0b,2b & 0b & 0b,2b & 0b & 0b,2b & 0b & 0b & & \\
 \hline \hline

\end{tabular}
}
\end{table}


==> tables/Intermediate_states.tex <==
%%%%%
%%%%%
%%%%%
\begin{table}[!ht]
\centering
\def\arraystretch{1.3}
    \caption{
        The most promising intermediate states for the considered \mHpp and \sina ranges, for \Hpp \Hmm pair, and  \Hpp \Hm, $H^0A^0$ associated productions 
    }
\label{tab:intermediate_charged}
\setlength{\tabcolsep}{0.0pc}
\resizebox{1\textwidth}{!}{
\begin{tabular}{ c | c  | c }
\hline \hline
Pair production & Associated production & Neutral  sector \\
%\hline \hline
% 4 W, 4W + 4Z, 6W + 2Z, 4b + 4W + 2Z, 6Z + 4W, 8W + 2Z (all masses) & 2Z+3W (all masses) & 1h + 3Z (all masses)  \\ 
%  6W + 2Z + 2b, 4W + 4Z + 2b, 6W + 4Z, 4W + 3Z + 2b (all masses)  & 5W (all masses) & 8W  (all masses)  \\ 
%8 W , 4W + 4Z + 1b , 6W + 1Z + 2b, 4W + 2b + 1Z ( 220 GeV )& 2b + 3W (all masses) &  4b + 4W (all masses)  \\
% 4W + 2b, 5W + 2b + 1Z, 7W + 1Z, 6W + 3Z (300 GeV)& 1h + %1Z + 3W (all masses) &  2b + 2W (220~GeV)   \\
%4W + 2 b + 1Z, 5Z + 4W, 8W + 4b, 6W + 6Z (300 GeV)  & 2b %+ 5W (400~GeV) & 2b + 2Z (220, 300~GeV)   \\
%400~GeV)& 1h + 1Z + 2W (220~GeV) \\
% 8b + 4W, 12W, 10W + 2Z, 10W + 2b, 8W + 4Z (300 GeV)  & 2h + 3W (300, 400~GeV) & 3h + Z (300~GeV)\\
%8W + 2Z + 2b, 6b + 4W + 4Z (300 GeV)&  & 2b + 2W + 2Z (400~GeV)  \\ 
%  8Z + 4W, 6W + 4Z + 2b,  6W + 2Z + 4b, 6W + 6b (300 GeV) &  &  2h + 4W (400~GeV)\\ 

\hline \hline
  4W, 4W + 3Z + 1h (all masses) & 3W+2Z, 3W + 3Z + 1h (all masses) & 1h + 3Z (all masses)  \\ 
   8W,  6 W + 2Z, 4W + 4b (220~GeV)  & 5W, 2b + 3W, 3W + 1Z + 1h (all masses) & 8W  (all masses)  \\ 
 4 W + 2b + 1h, 6W + 2b ( 220~GeV)& 7W, 3W + 2Z, 4W + 2Z, 3W +4b, 3W + 2Z + 2b  (220) &  4b + 4W (all masses)  \\
   4W + 2b + 2Z, 6W + 1h + 1Z  (220~GeV)& 3W + 2b + 1h + 1Z, 3W + 1Z + 2h, 5W + 1h + 1Z (220~GeV) &  2b + 2W (220~GeV)   \\
  4W + 4Z  (220, 300 GeV)  & 2b + 5W (220, 400~GeV) & 2b + 2Z (220, 300~GeV)   \\
   4W + 4h  (300 GeV)& 3W + 2Z + 2h (300~GeV) & 1h + 1Z + 2W (220~GeV) \\
   4W + 2Z + 2h, 4W + 3h + 1Z,1h + 3W, 2h + 3W  (300, 400 GeV)  & 4Z + 3W, 4h + 3W, 1h + 3W, 2h + 3W (300, 400~GeV)  & 3h + Z (300~GeV)\\
 8W + 4b, 6W + 1h + 1Z + 2b, 6W + 2b + 2Z (400 GeV)& 7W + 4b, 3W + 1Z + 1h, 5W + 2b + 1h + 1Z  (400~GeV)  & 2b + 2W + 2Z (400~GeV)  \\ 
   6W + 4b + 2h (400 GeV) & 3W + 2Z + 2h, 5W + 2b + 2h, 3W + 3h + 1Z, 3W + 2b 2Z (400~GeV )  &  2h + 4W (400~GeV)\\ 
 
 \hline \hline
\end{tabular}
}
\end{table}

==> tables/Neutral_finalstates.tex <==
%%%%%
%%%%%
%%%%%
\begin{table}[!ht]
\centering
\def\arraystretch{1.2}
\caption{ 
    The most promising final states for the neutral $H^{0} A^{0}$ associated production sector for $m_{H^{\pm \pm}} = 220, 300, 400$~GeV and  $\sin\alpha = $ $1 \times 10^{-4}$, $8 \times 10^{-4}$ and   $1.2 \times 10^{-3}$ values. 
}
\label{tab:neutral_finalstates}
\scalebox{0.61}{
\begin{tabular}{ c |c c c c c c c c c c c c  c c }
\hline \hline
& 2j & 2j+MET & 4j & 4j+MET & 6j & 6j+MET & 8j & 8j+MET & 10j & 10j+MET & 12j & 12j+MET & 14j  & 14j+MET \\
\hline
1l & & & & 2b & & 2b & &0b,2b,4b & & 2b, 4b & & 0b,2b & &0b \\
2l & & 2b & 2b & 2b & 2b, 6b & 0b,2b,4b & 0b,2b,4b & 2b,4b & 2b & 0b,2b & 0b,2b & 0b  & 0b & \\
3l & & & 0b,2b & 0b,4b & 0b,2b,4b &  & 0b,2b &  & 0b,2b & & & 0b & 0b & \\
4l  & 2b & 0b,2b & 2b & 0b,2b,4b & 0b,2b,4b & 0b,2b &  & 0b,2b & 0b,2b &  & 0b & & & \\
 \hline \hline
\end{tabular}
}
\end{table}
